QAFactEval: Improved QA-Based Factual Consistency Evaluation for Summarization

Factual consistency is an essential quality of text summarization models in practical settings. Existing work in evaluating this dimension can be broadly categorized into two lines of research, entailment-based and question answering (QA)-based metrics, and different experimental setups often lead to contrasting conclusions as to which paradigm performs the best. In this work, we conduct an extensive comparison of entailment and QA-based metrics, demonstrating that carefully choosing the components of a QA-based metric, especially question generation and answerability classification, is critical to performance. Building on those insights, we propose an optimized metric, which we call QAFactEval, that leads to a 14% average improvement over previous QA-based metrics on the SummaC factual consistency benchmark, and also outperforms the best-performing entailment-based metric. Moreover, we find that QA-based and entailment-based metrics can offer complementary signals and be combined into a single metric for a further performance boost.

==> 8-acknowledgements.tex <==
\section{Acknowledgements}\label{sec:acknowledgements}
We thank Philippe Laban for assistance in using the SummaC benchmark and SCConv model and for insightful discussions. 
We thank Wojciech Kry\'sci\'nski for assistance with editing the manuscript.

==> prev/6-analysis-discussion.tex <==
% \section{Analysis and Future Work}\label{sec:analysis-discussion}


==> prev/acl.tex <==
% % This must be in the first 5 lines to tell arXiv to use pdfLaTeX, which is strongly recommended.
% \pdfoutput=1
% % In particular, the hyperref package requires pdfLaTeX in order to break URLs across lines.

% \documentclass[11pt]{article}

% % Remove the "review" option to generate the final version.
% \usepackage[review]{acl}

% % Standard package includes
% \usepackage{times}
% \usepackage{latexsym}

% % For proper rendering and hyphenation of words containing Latin characters (including in bib files)
% \usepackage[T1]{fontenc}
% % For Vietnamese characters
% % \usepackage[T5]{fontenc}
% % See https://www.latex-project.org/help/documentation/encguide.pdf for other character sets

% % This assumes your files are encoded as UTF8
% \usepackage[utf8]{inputenc}

% % This is not strictly necessary, and may be commented out,
% % but it will improve the layout of the manuscript,
% % and will typically save some space.
% \usepackage{microtype}

% % If the title and author information does not fit in the area allocated, uncomment the following
% %
% %\setlength\titlebox{<dim>}
% %
% % and set <dim> to something 5cm or larger.

% \title{Instructions for *ACL Proceedings}

% % Author information can be set in various styles:
% % For several authors from the same institution:
% % \author{Author 1 \and ... \and Author n \\
% %         Address line \\ ... \\ Address line}
% % if the names do not fit well on one line use
% %         Author 1 \\ {\bf Author 2} \\ ... \\ {\bf Author n} \\
% % For authors from different institutions:
% % \author{Author 1 \\ Address line \\  ... \\ Address line
% %         \And  ... \And
% %         Author n \\ Address line \\ ... \\ Address line}
% % To start a seperate ``row'' of authors use \AND, as in
% % \author{Author 1 \\ Address line \\  ... \\ Address line
% %         \AND
% %         Author 2 \\ Address line \\ ... \\ Address line \And
% %         Author 3 \\ Address line \\ ... \\ Address line}

% \author{First Author \\
%   Affiliation / Address line 1 \\
%   Affiliation / Address line 2 \\
%   Affiliation / Address line 3 \\
%   \texttt{email@domain} \\\And
%   Second Author \\
%   Affiliation / Address line 1 \\
%   Affiliation / Address line 2 \\
%   Affiliation / Address line 3 \\
%   \texttt{email@domain} \\}

% \begin{document}
% \maketitle
% \begin{abstract}
% This document is a supplement to the general instructions for *ACL authors. It contains instructions for using the \LaTeX{} style files for ACL conferences. 
% The document itself conforms to its own specifications, and is therefore an example of what your manuscript should look like.
% These instructions should be used both for papers submitted for review and for final versions of accepted papers.
% \end{abstract}

% \section{Introduction}

% These instructions are for authors submitting papers to *ACL conferences using \LaTeX. They are not self-contained. All authors must follow the general instructions for *ACL proceedings,\footnote{\url{http://acl-org.github.io/ACLPUB/docs/formatting.html}} and this document contains additional instructions for the \LaTeX{} style files.

% The templates include the \LaTeX{} source of this document (\texttt{acl.tex}),
% the \LaTeX{} style file used to format it (\texttt{acl.sty}),
% an ACL bibliography style (\texttt{acl\_natbib.bst}),
% an example bibliography (\texttt{custom.bib}),
% and the bibliography for the ACL Anthology (\texttt{anthology.bib}).

% \section{Engines}

% To produce a PDF file, pdf\LaTeX{} is strongly recommended (over original \LaTeX{} plus dvips+ps2pdf or dvipdf). Xe\LaTeX{} also produces PDF files, and is especially suitable for text in non-Latin scripts.

% \section{Preamble}

% The first line of the file must be
% \begin{quote}
% \begin{verbatim}
% \documentclass[11pt]{article}
% \end{verbatim}
% \end{quote}

% To load the style file in the review version:
% \begin{quote}
% \begin{verbatim}
% \usepackage[review]{acl}
% \end{verbatim}
% \end{quote}
% For the final version, omit the \verb|review| option:
% \begin{quote}
% \begin{verbatim}
% \usepackage{acl}
% \end{verbatim}
% \end{quote}

% To use Times Roman, put the following in the preamble:
% \begin{quote}
% \begin{verbatim}
% \usepackage{times}
% \end{verbatim}
% \end{quote}
% (Alternatives like txfonts or newtx are also acceptable.)

% Please see the \LaTeX{} source of this document for comments on other packages that may be useful.

% Set the title and author using \verb|\title| and \verb|\author|. Within the author list, format multiple authors using \verb|\and| and \verb|\And| and \verb|\AND|; please see the \LaTeX{} source for examples.

% By default, the box containing the title and author names is set to the minimum of 5 cm. If you need more space, include the following in the preamble:
% \begin{quote}
% \begin{verbatim}
% \setlength\titlebox{<dim>}
% \end{verbatim}
% \end{quote}
% where \verb|<dim>| is replaced with a length. Do not set this length smaller than 5 cm.

% \section{Document Body}

% \subsection{Footnotes}

% Footnotes are inserted with the \verb|\footnote| command.\footnote{This is a footnote.}

% \subsection{Tables and figures}

% See Table~\ref{tab:accents} for an example of a table and its caption.
% \textbf{Do not override the default caption sizes.}

% \begin{table}
% \centering
% \begin{tabular}{lc}
% \hline
% \textbf{Command} & \textbf{Output}\\
% \hline
% \verb|{\"a}| & {\"a} \\
% \verb|{\^e}| & {\^e} \\
% \verb|{\`i}| & {\`i} \\ 
% \verb|{\.I}| & {\.I} \\ 
% \verb|{\o}| & {\o} \\
% \verb|{\'u}| & {\'u}  \\ 
% \verb|{\aa}| & {\aa}  \\\hline
% \end{tabular}
% \begin{tabular}{lc}
% \hline
% \textbf{Command} & \textbf{Output}\\
% \hline
% \verb|{\c c}| & {\c c} \\ 
% \verb|{\u g}| & {\u g} \\ 
% \verb|{\l}| & {\l} \\ 
% \verb|{\~n}| & {\~n} \\ 
% \verb|{\H o}| & {\H o} \\ 
% \verb|{\v r}| & {\v r} \\ 
% \verb|{\ss}| & {\ss} \\
% \hline
% \end{tabular}
% \caption{Example commands for accented characters, to be used in, \emph{e.g.}, Bib\TeX{} entries.}
% \label{tab:accents}
% \end{table}

% \subsection{Hyperlinks}

% Users of older versions of \LaTeX{} may encounter the following error during compilation: 
% \begin{quote}
% \tt\verb|\pdfendlink| ended up in different nesting level than \verb|\pdfstartlink|.
% \end{quote}
% This happens when pdf\LaTeX{} is used and a citation splits across a page boundary. The best way to fix this is to upgrade \LaTeX{} to 2018-12-01 or later.

% \subsection{Citations}

% \begin{table*}
% \centering
% \begin{tabular}{lll}
% \hline
% \textbf{Output} & \textbf{natbib command} & \textbf{Old ACL-style command}\\
% \hline
% \citep{Gusfield:97} & \verb|\citep| & \verb|\cite| \\
% \citealp{Gusfield:97} & \verb|\citealp| & no equivalent \\
% \citet{Gusfield:97} & \verb|\citet| & \verb|\newcite| \\
% \citeyearpar{Gusfield:97} & \verb|\citeyearpar| & \verb|\shortcite| \\
% \hline
% \end{tabular}
% \caption{\label{citation-guide}
% Citation commands supported by the style file.
% The style is based on the natbib package and supports all natbib citation commands.
% It also supports commands defined in previous ACL style files for compatibility.
% }
% \end{table*}

% Table~\ref{citation-guide} shows the syntax supported by the style files.
% We encourage you to use the natbib styles.
% You can use the command \verb|\citet| (cite in text) to get ``author (year)'' citations, like this citation to a paper by \citet{Gusfield:97}.
% You can use the command \verb|\citep| (cite in parentheses) to get ``(author, year)'' citations \citep{Gusfield:97}.
% You can use the command \verb|\citealp| (alternative cite without parentheses) to get ``author, year'' citations, which is useful for using citations within parentheses (e.g. \citealp{Gusfield:97}).

% \subsection{References}

% \nocite{Ando2005,borschinger-johnson-2011-particle,andrew2007scalable,rasooli-tetrault-2015,goodman-etal-2016-noise,harper-2014-learning}

% The \LaTeX{} and Bib\TeX{} style files provided roughly follow the American Psychological Association format.
% If your own bib file is named \texttt{custom.bib}, then placing the following before any appendices in your \LaTeX{} file will generate the references section for you:
% \begin{quote}
% \begin{verbatim}
% \bibliographystyle{acl_natbib}
% \bibliography{custom}
% \end{verbatim}
% \end{quote}

% You can obtain the complete ACL Anthology as a Bib\TeX{} file from \url{https://aclweb.org/anthology/anthology.bib.gz}.
% To include both the Anthology and your own .bib file, use the following instead of the above.
% \begin{quote}
% \begin{verbatim}
% \bibliographystyle{acl_natbib}
% \bibliography{anthology,custom}
% \end{verbatim}
% \end{quote}

% Please see Section~\ref{sec:bibtex} for information on preparing Bib\TeX{} files.

% \subsection{Appendices}

% Use \verb|\appendix| before any appendix section to switch the section numbering over to letters. See Appendix~\ref{sec:appendix} for an example.

% \section{Bib\TeX{} Files}
% \label{sec:bibtex}

% Unicode cannot be used in Bib\TeX{} entries, and some ways of typing special characters can disrupt Bib\TeX's alphabetization. The recommended way of typing special characters is shown in Table~\ref{tab:accents}.

% Please ensure that Bib\TeX{} records contain DOIs or URLs when possible, and for all the ACL materials that you reference.
% Use the \verb|doi| field for DOIs and the \verb|url| field for URLs.
% If a Bib\TeX{} entry has a URL or DOI field, the paper title in the references section will appear as a hyperlink to the paper, using the hyperref \LaTeX{} package.

% \section*{Acknowledgements}

% This document has been adapted
% by Steven Bethard, Ryan Cotterell and Rui Yan
% from the instructions for earlier ACL and NAACL proceedings, including those for 
% ACL 2019 by Douwe Kiela and Ivan Vuli\'{c},
% NAACL 2019 by Stephanie Lukin and Alla Roskovskaya, 
% ACL 2018 by Shay Cohen, Kevin Gimpel, and Wei Lu, 
% NAACL 2018 by Margaret Mitchell and Stephanie Lukin,
% Bib\TeX{} suggestions for (NA)ACL 2017/2018 from Jason Eisner,
% ACL 2017 by Dan Gildea and Min-Yen Kan, 
% NAACL 2017 by Margaret Mitchell, 
% ACL 2012 by Maggie Li and Michael White, 
% ACL 2010 by Jing-Shin Chang and Philipp Koehn, 
% ACL 2008 by Johanna D. Moore, Simone Teufel, James Allan, and Sadaoki Furui, 
% ACL 2005 by Hwee Tou Ng and Kemal Oflazer, 
% ACL 2002 by Eugene Charniak and Dekang Lin, 
% and earlier ACL and EACL formats written by several people, including
% John Chen, Henry S. Thompson and Donald Walker.
% Additional elements were taken from the formatting instructions of the \emph{International Joint Conference on Artificial Intelligence} and the \emph{Conference on Computer Vision and Pattern Recognition}.

% % Entries for the entire Anthology, followed by custom entries
% \bibliography{anthology,custom}
% \bibliographystyle{acl_natbib}

% \appendix

% \section{Example Appendix}
% \label{sec:appendix}

% This is an appendix.

% \end{document}

==> prev/helpers.tex <==

% % \begin{table}[t!]
% % \centering
% % \tiny
% % \resizebox{\columnwidth}{!}{\begin{tabular}{|l l c|}
% % \hline
% %     \textbf{Component}   & \textbf{Model Choice} &  \textbf{Benchmark}    \\ \hline
% %      \multirow{4}{*}{QAEval+}   &  AS: NP Chunks &  \multirow{4}{*}{79.5}   \\  
% %       & QG: BART-QA2D &  \\ 
% %       & QA: Electra-large &   \\ 
% %       & AO: LERC (ours) &   \\ \hline
% %     \multirow{3}{*}{Answer Selection}   &  Max NP &  77.1  \\  
% %       & NER     &  69.3  \\ 
% %       & ALL    & 78.3 \\ \hline
% %     \multirow{4}{*}{Question Generation}   &  BART-SQuAD &  76.6  \\  
% %       & T5-SQuAD     &  67.8  \\ 
% %       & MixQG-base    & 73.7   \\ 
% %       & MixQG-large   & 72.9  \\ \hline
% %     \multirow{3}{*}{Question Answering}   &  MADE &  77.9 \\  
% %     %   Electra-base   & 79.8   \\ \hline
% %       & \textit{T5}  &  77.7  \\ 
% %       & \textit{UnifiedQA}   & 78.5   \\ \hline
% %      \multirow{4}{*}{Answer Overlap}   &  EM &  72.2   \\  
% %       & F1 &   76.5  \\ 
% %       & Is\_answered &  75.9    \\ 
% %     %   & Is\_answered (T5) &   67.9  \\ 
% %       & LERC (orig) &  77.1    \\ \hline
% % %       LERC (BERT) &    77.1 \\ 
% % %       \hspace{15} (RoBERTa) & 80.0   \\ 
% % %       \hspace{15} (RoBERTa + QUIP) &   79.5 \\ \hline
% %       \multirow{3}{*}{Filtering/Answerability}  &  No QG Filter &  76.4   \\  
% %          & No Answerability &  74.9   \\  
% %           & No Filters &  71.6   \\  \hline
% % \end{tabular}}
% % \caption{Results of ablation studies on the validation set of the SummaC benchmark showing the effect of the individual components of QAEval+ on downstream factual consistency classification performance. \af{Will change structure of Table to make it clearer} }
% % \label{tab:ablation_all}
% % \end{table}
% % % Note from Alex: Updated the QG score since previous calculation excluded one of the benchmark datasets

% \newcommand{\AnswerExtractionAblation}{
% \begin{table}[t!]
% \centering
% \tiny
% \resizebox{.7\columnwidth}{!}{\begin{tabular}{|l|c|}
% \hline
%     \textbf{Model}   & \textbf{Benchmark}    \\ \hline
%       NP Chunks   &  79.5  \\ \hline
%       Max NP & 77.1 \\ \hline 
%       NER  &  69.3  \\ \hline
%       ALL   &  78.3  \\ \hline
% \end{tabular}}
% \caption{Effect of the type of answers extracted as input to conditional QG model on.}
% \label{tab:answer_extraction_ablation}
% \end{table}
% }
% % max-np: 0.771
% % all: 0.783
% % ner: 0.693
% % OG: 79.5

% \newcommand{\QGAblation}{
% \begin{table}[t!]
% \centering
% \tiny
% \resizebox{.85\columnwidth}{!}{\begin{tabular}{|l|c|}
% \hline
%     \textbf{Model}   & \textbf{Benchmark}    \\ \hline
%       BART-QA2D   &    79.5 \\ \hline
%       BART-SQuAD   &  76.6 \\ \hline
%       T5-SQuAD     &  67.8  \\ \hline
%       MixQG-base    & 69.5   \\ \hline
%       MixQG-large   & 70.5  \\ \hline
% \end{tabular}}
% \caption{Effect of varying QG model as well as finetuning QG dataset on factual consistency benchmark performance; results are on validation set. Doc refers to finetuning the QG model on data from \citet{demszky2018transforming}, while SQuAD refers to finetuning the QG model on SQuAD data \cite{rajpurkar-etal-2016-squad}.}
% \label{tab:qg_ablation}
% \end{table}
% }
% % AF: previously had T5-DOC in this but not including for now due to odd model outputs

% \newcommand{\QAAblation}{
% \begin{table}[t!]
% \centering
% \tiny
% \resizebox{.8\columnwidth}{!}{\begin{tabular}{|l|c|}
% \hline
%     \textbf{Model}   & \textbf{Benchmark}    \\ \hline
%       Electra-large   & 79.5   \\ \hline 
%     %   Electra-base   & 79.8   \\ \hline
%       MADE &    77.9 \\ \hline
%       \textit{T5-base}  &  77.7  \\ \hline
%       \textit{UnifiedQA-base}   & 78.5   \\ \hline
% \end{tabular}}
% \caption{Effect of varying QA model, including both extractive and abstractive (italicized). Other components, including question consistency and answerability classification, are held constant.}
% \label{tab:qa_ablation}
% \end{table}
% }
% % AF: leave question consistency from the original QA model - to discuss whether to change. 
% % AF: QuestEval has its own unanswerable classifier



% \newcommand{\AnswerabilityAblation}{
% \begin{table}[t!]
% \centering
% \tiny
% \resizebox{.8\columnwidth}{!}{\begin{tabular}{|l|c|}
% \hline
%     \textbf{Model}   & \textbf{Benchmark}    \\ \hline
%       Electra-large &  75.9  \\ \hline
%     %   Electra-base &  76.5  \\ \hline
%       T5 &   67.9  \\ \hline
% \end{tabular}}
% \caption{Effect of varying answerability classifier model, including taking answerability scores from the QA model. All models were trained on SQuAD.}
% \label{tab:ans_ablation}
% \end{table}
% }
% % 80.5 summeval try others
%     %   Electra-large-SQuAD-classifier &  \textcolor{red}{collecting}  \\ \hline
% % val for squad-classifier
% % 67.7 & 71.0 & 81.1 & 83.9 & 81.2 & 81.4 & 77.7
% % test for squad-classifier
% % 76.1 & 61.7 & 80.9 & 84.6 & 77.2 & 77.8 & 76.4


% \newcommand{\ConsAggAblation}{
% \begin{table}[t!]
% \centering
% \tiny
% \resizebox{\columnwidth}{!}{\begin{tabular}{|l|c|}
% \hline
%     \textbf{Model}   & \textbf{Benchmark}    \\ \hline
%       QAEval+ &  79.5  \\ \hline
%       \hspace{4} - Consistency &  76.4  \\ \hline
%       \hspace{4} - Answerability &  74.9  \\ \hline
%       \hspace{4} - Consistency \& Answerability &  71.6  \\ \hline
% \end{tabular}}
% \caption{Effect of filtering questions based on question consistency according to QA model. }
% \label{tab:cons_agg_ablation}
% \end{table}
% }
% % AF - will ignore aggregate for now since its contribution is not clear
% %   QA consistency + Aggregate &    \\ \hline
% %   W/Out QA consistency + Aggregate &    \\ \hline


% \newcommand{\LearnedMetricAblation}{
% \begin{table}[t!]
% \tiny
% \resizebox{\columnwidth}{!}{\begin{tabular}{|l|c|}
% \hline
%     \textbf{Model}   & \textbf{Benchmark}    \\ \hline
%       EM &  72.2  \\ \hline
%       F1 &   76.5 \\ \hline
%       Is\_answered &  75.9   \\ \hline
%       LERC (BERT) &    77.1 \\ 
%       \hspace{15} (RoBERTa) & 80.0   \\ 
%       \hspace{15} (RoBERTa + QUIP) &   79.5 \\ \hline
% \end{tabular}}
% \caption{Effect of answer overlap metric, including the effect of the choice of starting checkpoint for finetuned a learned answer overlap metric.}
% \label{tab:learned_metric_ablation}
% \end{table}
% }
% % Discuss difference when doing 5-fold CV: 72.9 for QUIP vs 72.7 for RoBERTa model




==> prev/prev_intro.tex <==

% Copy of above
% Our contributions are the following: 
% 1) We analyze all components of the QA-based metric pipeline, highlighting the current model bottleneck in question generation and answerability classification. 
% % 
% 2) We improve performance over previous QA-based metrics by over 15\% on a factual consistency benchmark consisting of 6 individual datasets, achieving state-of-the-art results. \wojciech{<- Should this be point 2)?} \af{Agree it does suggest a separate bullet point as currently written - may come back}
% 3) We show that QA-based metrics and NLI-based metrics offer complementary signals and combine them in a new metric through a simple learned network, further improving evaluation performance. 
% 4) We report results for 10 additional metrics across binary classification and correlation analysis, providing the most comprehensive benchmark results for factual consistency metrics~\footnote{Code and checkpoints will be made publicly available: \url{https://github.com/salesforce/QAFactEval}}. 
% % perform a qualitative analysis of our model outputs and - \af{not really true - qualitative analysis is more in}


% \input{tables/example_intro}
% \section{Introduction}\label{sec:introduction}
% Text summarization aims to compress long document(s) into a short and fluent form that preserves salient information. 
% % 
% Recent neural models have made extensive gains in NLP, especially through advances in pretrained language models such as BERT~\cite{devlin-etal-2019-bert}, which have motivated a shift to pretraining methods in summarization~\interalia{liu-lapata-2019-text,lewis2019bart,zhang2019pegasus}.
% % 
% % \citep{liu-lapata-2019-text, zhang-etal-2019-hibert, dong2019unified, ziegler2019fine, 2019t5, lewis2019bart}. 
% % 
% However, despite recent improvements on datasets such as CNN/DailyMail \cite{hermann2015teaching} and XSum \cite{xsum-emnlp}, state-of-the-art models and are not always factually consistent with the source documents upon which they are conditioned on~\interalia{maynez-etal-2020-faithfulness,fabbri2021summeval}. 
% Thus, determining the factual consistency of a summary remains an essential task.
% % as a means of improving model training and determining the usability of such models. \af{include or not?}
% \par 
% % 
% Recent metrics for summarization factual consistency can be broadly split into two categories 
% % 
% 1) Embedding and entailment models which compute an embedding similarity or entailment relationship between the source document(s) and summary \interalia{kryscinskiFactCC2019,DBLP:journals/corr/abs-2011-13662} and 
% % 
% 2) QA-based models, which first phrases from the summary, generate questions for these phrases using a question generation (QG) model and compute a factual consistency score based on a QA model's ability to answer these questions, typically using the source document as context, \interalia{deutsch2020questionanswering,scialom2020QuestEval}. 
% % 
% % 
% We provide an illustrative example in Table \ref{tab:example_intro} in which both metrics correctly identify the factual inconsistency and output a low score. 
% % 
% While entailment-based methods intuitively measure information in the summary supported by the source document, QA-based metrics have been shown to more precisely measure information overlap \cite{deutsch-roth-2021-understanding} and consist of a pipeline with easily-understood component outputs. % 
% % 
% % 

% Comparisons among entailment-based and QA-based metrics, however, often differ in their choice of baseline model and input granularity, evaluating on single datasets and drawing differing conclusions as to the best paradigm. 
% For example, some work reports entailment-based metrics as performing baest \citet{DBLP:journals/corr/abs-2004-04228,maynez-etal-2020-faithfulness,DBLP:journals/corr/abs-2004-04228}, while other work argues for QA metrics as state-of-the-art \citet{durmus-etal-2020-feqa,wang-etal-2020-asking,scialom2020QuestEval}.
% % 
% % 
% Recently, \citet{laban2021summac} proposed a benchmark called \textit{SummaC} to compare metrics across six factual consistency datasets for the task of binary factual consistency classification, whether a summary is entirely factually consistent or not. 
% This work unifies prior work on entailment-based metrics by studying the effect of input granularity, pretrained entailment model, and other hyperparameter choices on downstream evaluation performance. 
% % 
% However, that work does not study the components of QA-based metrics. 
% \par
% In order to unify work in QA-based factual consistency evaluation, we do an extensive hyperparameter analysis of current metrics. 
% We break down these metrics into four constituent components, namely the selection of answers to ask questions about, question generation (QG) conditioned upon these answers, question answering based on the source document, and answer overlap evaluation between model and reference answers. 
% We show that by correctly optimizing each of these components, our proposed QA-based metric, which we call \qafacteval~ outperforms the entailment-based metrics of \citet{laban2021summac}.

% Our contributions are the following: 
% 1) We analyze all components of the QA-based metric pipeline, determining the current model bottleneck in question generation and answerability classification. 
% We improve performance over previous QA-based metrics by over 15\% on a factual consistency benchmark consisting of 6 individual datasets, achieving state-of-the-art results. 
% 2) We show that QA-based metrics and NLI-based metrics offer complementary signals and combine them in a new metric through a simple learned network, further improving evaluation performance. 
% 3) We perform a qualitative analysis of our model outputs and report results for 10 additional metrics across binary classification and correlation analysis, providing the most comprehensive benchmark results for factual consistency metrics~\footnote{Code and checkpoints will be made publicly available: \url{https://github.com/salesforce/QAFactEval}}.
% %  \footnote{For reproducibility of our findings, we will make our data and code publicly available at \url{https://github.com/TODO}.}
% % \af{Mentioned SummaC explicitly}

==> prev/prev_misc.tex <==
% 
% Evaluation metric comparisons for factual consistency in summarization often vary in their choice of baselines and model parameters, leading to differing conclusions as to which metric truly performs best. 
% Entailment-based metrics measure factual consistency based on the factual support of the summary found in the input, while Question-answering (QA)-based metrics measure the answerability, using the input document(s) as context, of questions generated from the summary.
% % ~\jason{Missing one sentence to introduce entailment-based and QA-based solutions and connect to the next sentence.} % ~\jason{We can directly cite the work} 
% \citet{laban2021summac} show that correctly optimizing the parameters of entailment-based evaluation metrics greatly improves factual consistency evaluation performance.
% % 
% In this work, we demonstrate that carefully choosing the components of QA-based metrics is critical to performance, leading to over a 15\% improvement over previous QA-based metrics on the task of binary factual consistency classification and outperforming optimized entailment-based metrics by about 5\%. 
% Furthermore, we observe that QA and entailment-based metrics offer complimentary signals and can be combined for a further performance boost. 
% % 
% Our qualitative analysis and experiments on both factual consistency classification and correlation tasks identify question generation and answer overlap evaluation as critical components of the QA metric pipeline upon which future work may improve. 
% answerability classification and producing finer-grained question-answering metric evaluations as directions for future work~
% \jason{I would rather add some takeaway or insights here}. \alex{added temporary; will update.}

==> prev/prev_related_work.tex <==
% \section{Related Work}\label{sec:related-work}
% \paragraph{Evaluating Factual Consistency}
% Within entailment-based factual consistency evaluation,
% % 
% % , entailment-based metrics have received much attention due to the similarities between the two tasks ;
% % 
% % A summary should show support or be neutral to the input source. 
% % 
% \citet{falke-etal-2019-ranking} propose the task of ranking summary pairs for factual consistency based on entailment models and release a set of 379 summary pairs, while
% \citet{kryscinskiFactCC2019} explore factual consistency classification jointly with source support or contradiction span extraction. 
% % identify whether sentences remain factually consistent after transformation,
% % extract a span in the source documents to support the consistency prediction,
% % 
% % \wojciech{Why no love for FactCC and the source attribution/error highlighting mechanism ;(} \af{added - will reword :)}
% % 
% % \citet{poliak-2020-survey}  provide a survey for using entailment-based models as evaluation metrics. 
% % 
% Other work on factual consistency and entailment has examined input granularity \cite{goyal-durrett-2020-evaluating},
% compared adversarial learning for entailment models \cite{Barrantes2020AdversarialNF}, and explored the use of entailment-based models as the backbone of others metrics such as BERTScore \cite{bert-score} as in \citet{koto2021ffci}. 
% % 
% % While favorable correlations between entailment models and faithfulness \cite{maynez-etal-2020-faithfulness}, m
% Metric comparisons, however, were often conducted on isolated datasets. 
% % 
% \citet{laban2021summac} unify work in entailment-based metrics for factual consistency, showing the effect of granularity, base models, and other hyperparameter choices.
% % 
% This work also proposes a learned metric built on top of the output of an entailment model, with parameters fine-tuned on synthetic data.
% %
% While this work fills a gap in the use of entailment-based metrics for factual consistency, our work analogously unifies QA-based metrics for factual consistency and proposes to combine entailment and QA-based metrics in a single learned metric.
% % \af{position our paper}
% % 
% \par
% Another line of work in factual consistency evaluation centers around  QA-based metrics \cite{scialom-etal-2019-answers,durmus-etal-2020-feqa,wang-etal-2020-asking,scialom2020QuestEval,deutsch2020questionanswering}.
% Recent work has shown that QA-based metrics better measure the overlap of information units for determining summary relevance over embedding-based metrics metrics \cite{deutsch-roth-2021-understanding}, further driving our study of QA-based metrics for factual consistency. 
% % 
% % QA-based metrics for factual consistency operate under the assumption that the ability of a QA model to answer questions, typically generated from the summary, using the input as context. 
% % 
% % However, these models differ in underlying answer selection, question generation, question answering and answer overlap components.
% % 
% While several QA-based models with similar structure have been applied for factual consistency,
% \cite{durmus-etal-2020-feqa,wang-etal-2020-asking,scialom2020QuestEval}, they differ in their underlying answer selection, question generation, question answering and answer overlap components, reporting different performances.
% % 
% % and do not report results across many datasets. 
% % 
% In our work, we perform a comprehensive evaluation of QA-based metric components and propose improved model components for the task of answer overlap and question consistency. 
% % 
% % 
% \paragraph{Summarization Benchmarking}
% With the introduction of pretrained models that have achieved state-of-the-art performance across many datasets, a recent line of work aims to take stock of the current state of summarization models and progress, both within factual consistency and across summarization more broadly.
% % 
% \citet{kryscinski-critical-eval} note biases and failure modes of abstractive summarization models, while other work analyzes and collect annotations over the output of recent summarization models across multiple dimensions, including factual consistency \citet{fabbri2021summeval,Bhandari-2020-reevaluating,huang-etal-2020-achieved}. 
% % 
% \citet{lux-etal-2020-truth} propose a typology of errors found in summarization models, while \citet{gabriel-etal-2021-go} propose a framework for meta-evaluation of faithfulness consistency metrics. \citet{laban2021summac} propose to combine recent work in factual consistency evaluation for summarization through a single benchmark, SummaC and optimize entailment-based evaluation metrics. 
% % 
% Our work directly makes use of this benchmark while emphasizing QA-based metrics. 
% % We also include correlation analysis for a more comprehensive understanding of current factual consistency metrics. 
